Structural Pruning of Pre-trained Language Models via Neural Architecture Search

Pre-trained language models (PLM), for example BERT or RoBERTa, mark the state-of-the-art for natural language understanding task when fine-tuned on labeled data. However, their large size poses challenges in deploying them for inference in real-world applications, due to significant GPU memory requirements and high inference latency. This paper explores neural architecture search (NAS) for structural pruning to find sub-parts of the fine-tuned network that optimally trade-off efficiency, for example in terms of model size or latency, and generalization performance. We also show how we can utilize more recently developed two-stage weight-sharing NAS approaches in this setting to accelerate the search process. Unlike traditional pruning methods with fixed thresholds, we propose to adopt a multi-objective approach that identifies the Pareto optimal set of sub-networks, allowing for a more flexible and automated compression process.

==> figures/docs/17a14533-ba9f-451c-873c-ac38f6314cc3 <==
{"id":"321241621323","lines":[{"id":"n0.8769566614754446","blocks":[],"style":{"align":"center"}},{"id":"n0.13767869811611155","blocks":[],"style":{"align":"center"}},{"id":"n0.9077422112594957","blocks":[],"style":{"align":"center"}},{"id":"n0.1385238851042523","blocks":[],"style":{"align":"center"}},{"id":"n0.2704574344403258","blocks":[{"id":"n0.5608184816006905","text":"\\diagram","type":"composite","elements":{"de15872564412344636":{"id":"de15872564412344636","lines":[{"id":"n0.5351898422389241","blocks":[{"id":"n0.6753205895720424","text":"FFN Layer"}]}],"shape":{"data":{"p":{"x":10,"y":5}},"anchor":"left-top"},"isTextMode":true},"de22580378445063232":{"id":"de22580378445063232","lines":[{"blocks":[{"text":"MHA Layer","id":"n0.33533794957166474"}],"id":"n0.41455719693878335"}],"shape":{"data":{"p":{"x":10,"y":40}},"anchor":"left-top"},"isTextMode":true},"de407714988560147":{"id":"de407714988560147","lines":[{"blocks":[{"text":"FFN Layer","id":"n0.7488330767546975"}],"id":"n0.23234752782950585"}],"shape":{"data":{"p":{"x":10,"y":81}},"anchor":"left-top"},"isTextMode":true},"de807510991842164":{"id":"de807510991842164","lines":[{"blocks":[{"text":"MHA Layer","id":"n0.8488426865466416"}],"id":"n0.947631308471787"}],"shape":{"data":{"p":{"x":10,"y":120}},"anchor":"left-top"},"isTextMode":true},"de8423373323094074":{"id":"de8423373323094074","lines":[{"blocks":[{"text":"FFN Layer","id":"n0.17666807604571555"}],"id":"n0.965374470354247"}],"shape":{"data":{"p":{"x":10,"y":160}},"anchor":"left-top"},"isTextMode":true},"de8090420777618776":{"id":"de8090420777618776","lines":[{"blocks":[{"text":"MHA Layer","id":"n0.5844170406581082"}],"id":"n0.620898928370131"}],"shape":{"data":{"p":{"x":10,"y":200}},"anchor":"left-top"},"isTextMode":true},"de30984490567439205":{"id":"de30984490567439205","lines":[{"blocks":[{"text":"FFN Layer","id":"n0.23054050367025503"}],"id":"n0.6964567105676739"}],"shape":{"data":{"p":{"x":10,"y":240}},"anchor":"left-top"},"isTextMode":true},"de8267892635353894":{"id":"de8267892635353894","lines":[{"blocks":[{"text":"MHA Layer","id":"n0.2592974597116997"}],"id":"n0.025955210192152967"}],"shape":{"data":{"p":{"x":10,"y":280}},"anchor":"left-top"},"isTextMode":true},"de6881830168375056":{"id":"de6881830168375056","lines":[{"blocks":[{"text":"FFN Mask","id":"n0.541978367060488"}],"id":"n0.41901437205880376"}],"shape":{"data":{"p":{"x":361,"y":-3}},"anchor":"left-top"},"isTextMode":true},"de9239778778426443":{"id":"de9239778778426443","lines":[{"blocks":[{"text":"MHA Mask","id":"n0.33285322041010845"}],"id":"n0.42247066379905773"}],"shape":{"data":{"p":{"x":358,"y":274}},"anchor":"left-top"},"isTextMode":true},"de2385546399661993":{"id":"de2385546399661993","lines":[{"id":"n0.7335375491202799","blocks":[{"id":"n0.6021284722791883","text":"x","style":{"fontSize":"\\Large"}}]}],"shape":{"data":{"p":{"x":305,"y":65.5}},"anchor":"left-top"},"isTextMode":true},"de7170527458811329":{"id":"de7170527458811329","lines":[{"blocks":[{"text":"x","style":{"fontSize":"\\Large"},"id":"n0.5314155618670479"}],"id":"n0.929564768281507"}],"shape":{"data":{"p":{"x":300,"y":192.5}},"anchor":"left-top"},"isTextMode":true},"de3749512747515755":{"id":"de3749512747515755","lines":[{"blocks":[{"id":"n0.9575187632303573","text":"Pre-Trained Network"}],"id":"n0.8363715416925682"}],"shape":{"data":{"p":{"x":118,"y":318}},"anchor":"left-top"},"isTextMode":true},"de6027206310748856":{"id":"de6027206310748856","lines":[{"blocks":[{"text":"Sub-Network","id":"n0.5433266089029549"}],"id":"n0.9639269770951215"}],"shape":{"data":{"p":{"x":525,"y":315}},"anchor":"left-top"},"isTextMode":true}},"connections":[],"intersections":{"id":"di9799532208962962","items":[],"style":{}},"shapes":[{"id":"dg8444052064779246","entities":[{"id":"dp11760701084601433","type":"rectangle","data":{"p1":{"x":120,"y":40},"p2":{"x":270,"y":65.5}},"style":{"fillColor":[184,233,134,1]}},{"id":"dp4747712256132679","type":"rectangle","data":{"p1":{"x":120,"y":0},"p2":{"x":270,"y":25.5}},"style":{"fillColor":[120,164,216,1]}},{"id":"dp2438406175254234","type":"rectangle","data":{"p1":{"x":120,"y":80},"p2":{"x":270,"y":105.5}},"style":{"fillColor":[120,164,216,1]}},{"id":"dp5890302888764098","type":"rectangle","data":{"p1":{"x":120,"y":120},"p2":{"x":270,"y":145.5}},"style":{"fillColor":[184,233,134,1]}},{"id":"dp9432636726993874","type":"rectangle","data":{"p1":{"x":120,"y":200},"p2":{"x":270,"y":225.5}},"style":{"fillColor":[184,233,134,1]}},{"id":"dp5282732584540336","type":"rectangle","data":{"p1":{"x":120,"y":160},"p2":{"x":270,"y":185.5}},"style":{"fillColor":[120,164,216,1]}},{"id":"dp5305938529109827","type":"rectangle","data":{"p1":{"x":120,"y":240},"p2":{"x":270,"y":265.5}},"style":{"fillColor":[120,164,216,1]}},{"id":"dp7832146899175839","type":"rectangle","data":{"p1":{"x":120,"y":280},"p2":{"x":270,"y":305.5}},"style":{"fillColor":[184,233,134,1]}}]},{"id":"dg23724562693103812","entities":[{"id":"dp04218687518383346","type":"rectangle","data":{"p1":{"x":500,"y":41},"p2":{"x":650,"y":66.5}},"style":{"fillColor":[184,233,134,1]}},{"id":"dp4051637753867142","type":"rectangle","data":{"p1":{"x":499,"y":0},"p2":{"x":649,"y":25.5}},"style":{"fillColor":[120,164,216,1]}},{"id":"dp39507965521995014","type":"rectangle","data":{"p1":{"x":499,"y":200},"p2":{"x":649,"y":225.5}},"style":{"fillColor":[184,233,134,1]}},{"id":"dp13209930708385909","type":"rectangle","data":{"p1":{"x":499,"y":240},"p2":{"x":649,"y":265.5}},"style":{"fillColor":[120,164,216,1]}},{"id":"dp6469043741338977","type":"rectangle","data":{"p1":{"x":499,"y":280},"p2":{"x":649,"y":305.5}},"style":{"fillColor":[184,233,134,1]}},{"id":"dp18217977992914192","type":"rectangle","data":{"p1":{"x":609,"y":280},"p2":{"x":650,"y":305.5}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp9547796103351931","type":"rectangle","data":{"p1":{"x":500,"y":81},"p2":{"x":650,"y":106.5}},"style":{"fillColor":[120,164,216,1]}},{"id":"dp023334165472781998","type":"rectangle","data":{"p1":{"x":500,"y":121},"p2":{"x":650,"y":146.5}},"style":{"fillColor":[184,233,134,1]}},{"id":"dp18426378660141263","type":"rectangle","data":{"p1":{"x":500,"y":161},"p2":{"x":650,"y":186.5}},"style":{"fillColor":[120,164,216,1]}},{"id":"dp2380834684119021","type":"rectangle","data":{"p1":{"x":562,"y":0},"p2":{"x":649,"y":25.5}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp4155092640993481","type":"rectangle","data":{"p1":{"x":563,"y":81},"p2":{"x":650,"y":106.5}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp2972421551193586","type":"rectangle","data":{"p1":{"x":563,"y":161},"p2":{"x":650,"y":186.5}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp719665246497301","type":"rectangle","data":{"p1":{"x":562,"y":240},"p2":{"x":649,"y":265.5}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp010085662675391682","type":"rectangle","data":{"p1":{"x":609,"y":41},"p2":{"x":650,"y":66.5}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp6400198248521445","type":"rectangle","data":{"p1":{"x":609,"y":121},"p2":{"x":650,"y":146.5}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp4273263436161897","type":"rectangle","data":{"p1":{"x":608,"y":200},"p2":{"x":649,"y":225.5}},"style":{"fillColor":[255,255,255,1]}}]},{"id":"dg020105370679470935","entities":[{"id":"dp9998757183243281","type":"rectangle","data":{"p1":{"x":347,"y":163},"p2":{"x":357,"y":173},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp02464604220966171","type":"rectangle","data":{"p1":{"x":357,"y":163},"p2":{"x":367,"y":173},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp5854771734651532","type":"rectangle","data":{"p1":{"x":367,"y":163},"p2":{"x":377,"y":173},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp5441589462990419","type":"rectangle","data":{"p1":{"x":377,"y":163},"p2":{"x":387,"y":173},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp46419649525156714","type":"rectangle","data":{"p1":{"x":387,"y":163},"p2":{"x":397,"y":173},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp8383908969613525","type":"rectangle","data":{"p1":{"x":397,"y":163},"p2":{"x":407,"y":173},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp6406634307603872","type":"rectangle","data":{"p1":{"x":407,"y":163},"p2":{"x":417,"y":173},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp3822074460151348","type":"rectangle","data":{"p1":{"x":417,"y":163},"p2":{"x":427,"y":173},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp6047613495315152","type":"rectangle","data":{"p1":{"x":427,"y":163},"p2":{"x":437,"y":173},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp6660534488877469","type":"rectangle","data":{"p1":{"x":437,"y":163},"p2":{"x":447,"y":173},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dg9451734303732344","entities":[{"id":"dp2938942927406798","type":"rectangle","data":{"p1":{"x":347,"y":173},"p2":{"x":357,"y":183},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp2864393192600616","type":"rectangle","data":{"p1":{"x":357,"y":173},"p2":{"x":367,"y":183},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp036684320859258435","type":"rectangle","data":{"p1":{"x":367,"y":173},"p2":{"x":377,"y":183},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp7068424376693963","type":"rectangle","data":{"p1":{"x":377,"y":173},"p2":{"x":387,"y":183},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp01155887230029129","type":"rectangle","data":{"p1":{"x":387,"y":173},"p2":{"x":397,"y":183},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp17164293591994917","type":"rectangle","data":{"p1":{"x":397,"y":173},"p2":{"x":407,"y":183},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp3181024282493006","type":"rectangle","data":{"p1":{"x":407,"y":173},"p2":{"x":417,"y":183},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp46865116784238914","type":"rectangle","data":{"p1":{"x":417,"y":173},"p2":{"x":427,"y":183},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp4422932642613081","type":"rectangle","data":{"p1":{"x":427,"y":173},"p2":{"x":437,"y":183},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp9148207170925569","type":"rectangle","data":{"p1":{"x":437,"y":173},"p2":{"x":447,"y":183},"flipX":true},"style":{"fillColor":[184,233,134,1]}}]},{"id":"dg12313645372359394","entities":[{"id":"dp11232447450539906","type":"rectangle","data":{"p1":{"x":347,"y":183},"p2":{"x":357,"y":193},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp7000023370263986","type":"rectangle","data":{"p1":{"x":357,"y":183},"p2":{"x":367,"y":193},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp6265545736606314","type":"rectangle","data":{"p1":{"x":367,"y":183},"p2":{"x":377,"y":193},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp26608832273188154","type":"rectangle","data":{"p1":{"x":377,"y":183},"p2":{"x":387,"y":193},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp4562764071934703","type":"rectangle","data":{"p1":{"x":387,"y":183},"p2":{"x":397,"y":193},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp8152137979990752","type":"rectangle","data":{"p1":{"x":397,"y":183},"p2":{"x":407,"y":193},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp4568003280355065","type":"rectangle","data":{"p1":{"x":407,"y":183},"p2":{"x":417,"y":193},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp751932568856875","type":"rectangle","data":{"p1":{"x":417,"y":183},"p2":{"x":427,"y":193},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp9162401754560425","type":"rectangle","data":{"p1":{"x":427,"y":183},"p2":{"x":437,"y":193},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp6035531571478931","type":"rectangle","data":{"p1":{"x":437,"y":183},"p2":{"x":447,"y":193},"flipX":true},"style":{"fillColor":[184,233,134,1]}}]},{"id":"dg5371619184733077","entities":[{"id":"dp7293588594329284","type":"rectangle","data":{"p1":{"x":347,"y":193},"p2":{"x":357,"y":203},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp10238661975410479","type":"rectangle","data":{"p1":{"x":357,"y":193},"p2":{"x":367,"y":203},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp9303470026468514","type":"rectangle","data":{"p1":{"x":367,"y":193},"p2":{"x":377,"y":203},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp11403091639938878","type":"rectangle","data":{"p1":{"x":377,"y":193},"p2":{"x":387,"y":203},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp10926602487526715","type":"rectangle","data":{"p1":{"x":387,"y":193},"p2":{"x":397,"y":203},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp5955027204809126","type":"rectangle","data":{"p1":{"x":397,"y":193},"p2":{"x":407,"y":203},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp6867004821298737","type":"rectangle","data":{"p1":{"x":407,"y":193},"p2":{"x":417,"y":203},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp190110365187103","type":"rectangle","data":{"p1":{"x":417,"y":193},"p2":{"x":427,"y":203},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp6678413364252953","type":"rectangle","data":{"p1":{"x":427,"y":193},"p2":{"x":437,"y":203},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp6179437774513415","type":"rectangle","data":{"p1":{"x":437,"y":193},"p2":{"x":447,"y":203},"flipX":true},"style":{"fillColor":[184,233,134,1]}}]},{"id":"dg9702688171925677","entities":[{"id":"dp23798980910569523","type":"rectangle","data":{"p1":{"x":347,"y":203},"p2":{"x":357,"y":213},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp06312799829619309","type":"rectangle","data":{"p1":{"x":357,"y":203},"p2":{"x":367,"y":213},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp4991167727168625","type":"rectangle","data":{"p1":{"x":367,"y":203},"p2":{"x":377,"y":213},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp4047413340556407","type":"rectangle","data":{"p1":{"x":377,"y":203},"p2":{"x":387,"y":213},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp8843302831692738","type":"rectangle","data":{"p1":{"x":387,"y":203},"p2":{"x":397,"y":213},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp8079600149945096","type":"rectangle","data":{"p1":{"x":397,"y":203},"p2":{"x":407,"y":213},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp5728520461272346","type":"rectangle","data":{"p1":{"x":407,"y":203},"p2":{"x":417,"y":213},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp6124374838174047","type":"rectangle","data":{"p1":{"x":417,"y":203},"p2":{"x":427,"y":213},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp2798746379499686","type":"rectangle","data":{"p1":{"x":427,"y":203},"p2":{"x":437,"y":213},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp6298321442255035","type":"rectangle","data":{"p1":{"x":437,"y":203},"p2":{"x":447,"y":213},"flipX":true},"style":{"fillColor":[184,233,134,1]}}]},{"id":"dg6741724391041864","entities":[{"id":"dp8155767888400357","type":"rectangle","data":{"p1":{"x":347,"y":213},"p2":{"x":357,"y":223},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp2193002908453594","type":"rectangle","data":{"p1":{"x":357,"y":213},"p2":{"x":367,"y":223},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp4269530195465542","type":"rectangle","data":{"p1":{"x":367,"y":213},"p2":{"x":377,"y":223},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp3880148702477719","type":"rectangle","data":{"p1":{"x":377,"y":213},"p2":{"x":387,"y":223},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp48722077431509214","type":"rectangle","data":{"p1":{"x":387,"y":213},"p2":{"x":397,"y":223},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp4842584876808126","type":"rectangle","data":{"p1":{"x":397,"y":213},"p2":{"x":407,"y":223},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp8391801459152133","type":"rectangle","data":{"p1":{"x":407,"y":213},"p2":{"x":417,"y":223},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp9886393462149489","type":"rectangle","data":{"p1":{"x":417,"y":213},"p2":{"x":427,"y":223},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp8695063443113497","type":"rectangle","data":{"p1":{"x":427,"y":213},"p2":{"x":437,"y":223},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp1795442021090835","type":"rectangle","data":{"p1":{"x":437,"y":213},"p2":{"x":447,"y":223},"flipX":true},"style":{"fillColor":[184,233,134,1]}}]},{"id":"dg4718497464079011","entities":[{"id":"dp24242368550115712","type":"rectangle","data":{"p1":{"x":347,"y":223},"p2":{"x":357,"y":233},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp5743489053117228","type":"rectangle","data":{"p1":{"x":357,"y":223},"p2":{"x":367,"y":233},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp6059956785354248","type":"rectangle","data":{"p1":{"x":367,"y":223},"p2":{"x":377,"y":233},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp7340724871342698","type":"rectangle","data":{"p1":{"x":377,"y":223},"p2":{"x":387,"y":233},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp9448297880046023","type":"rectangle","data":{"p1":{"x":387,"y":223},"p2":{"x":397,"y":233},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp9949604396566202","type":"rectangle","data":{"p1":{"x":397,"y":223},"p2":{"x":407,"y":233},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp33700945474188704","type":"rectangle","data":{"p1":{"x":407,"y":223},"p2":{"x":417,"y":233},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp3047361164035832","type":"rectangle","data":{"p1":{"x":417,"y":223},"p2":{"x":427,"y":233},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp11401546466043788","type":"rectangle","data":{"p1":{"x":427,"y":223},"p2":{"x":437,"y":233},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp9571445148201243","type":"rectangle","data":{"p1":{"x":437,"y":223},"p2":{"x":447,"y":233},"flipX":true},"style":{"fillColor":[184,233,134,1]}}]},{"id":"dg47112418554233304","entities":[{"id":"dp9592292690817065","type":"rectangle","data":{"p1":{"x":347,"y":233},"p2":{"x":357,"y":243},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp43366201416303685","type":"rectangle","data":{"p1":{"x":357,"y":233},"p2":{"x":367,"y":243},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp7694064473107137","type":"rectangle","data":{"p1":{"x":367,"y":233},"p2":{"x":377,"y":243},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp19702774238248322","type":"rectangle","data":{"p1":{"x":377,"y":233},"p2":{"x":387,"y":243},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp49679136058839346","type":"rectangle","data":{"p1":{"x":387,"y":233},"p2":{"x":397,"y":243},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp799434695387416","type":"rectangle","data":{"p1":{"x":397,"y":233},"p2":{"x":407,"y":243},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp28108214368710216","type":"rectangle","data":{"p1":{"x":407,"y":233},"p2":{"x":417,"y":243},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp7592068720340772","type":"rectangle","data":{"p1":{"x":417,"y":233},"p2":{"x":427,"y":243},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp6586177409267692","type":"rectangle","data":{"p1":{"x":427,"y":233},"p2":{"x":437,"y":243},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp7304088737153395","type":"rectangle","data":{"p1":{"x":437,"y":233},"p2":{"x":447,"y":243},"flipX":true},"style":{"fillColor":[184,233,134,1]}}]},{"id":"dg44479364430093193","entities":[{"id":"dp05870558975517104","type":"rectangle","data":{"p1":{"x":347,"y":243},"p2":{"x":357,"y":253},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp5439646608880496","type":"rectangle","data":{"p1":{"x":357,"y":243},"p2":{"x":367,"y":253},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp4250788547630956","type":"rectangle","data":{"p1":{"x":367,"y":243},"p2":{"x":377,"y":253},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp19871601477256673","type":"rectangle","data":{"p1":{"x":377,"y":243},"p2":{"x":387,"y":253},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp17439884535764427","type":"rectangle","data":{"p1":{"x":387,"y":243},"p2":{"x":397,"y":253},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp22391072484191588","type":"rectangle","data":{"p1":{"x":397,"y":243},"p2":{"x":407,"y":253},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp6217066793197638","type":"rectangle","data":{"p1":{"x":407,"y":243},"p2":{"x":417,"y":253},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp5967833225179269","type":"rectangle","data":{"p1":{"x":417,"y":243},"p2":{"x":427,"y":253},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp6002807238298143","type":"rectangle","data":{"p1":{"x":427,"y":243},"p2":{"x":437,"y":253},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp35418996133580305","type":"rectangle","data":{"p1":{"x":437,"y":243},"p2":{"x":447,"y":253},"flipX":true},"style":{"fillColor":[184,233,134,1]}}]},{"id":"dg861007564753931","entities":[{"id":"dp0436715479203833","type":"rectangle","data":{"p1":{"x":347,"y":253},"p2":{"x":357,"y":263},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp9033737646172075","type":"rectangle","data":{"p1":{"x":357,"y":253},"p2":{"x":367,"y":263},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp3518169597149816","type":"rectangle","data":{"p1":{"x":367,"y":253},"p2":{"x":377,"y":263},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp8485002589625444","type":"rectangle","data":{"p1":{"x":377,"y":253},"p2":{"x":387,"y":263},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp304890482733984","type":"rectangle","data":{"p1":{"x":387,"y":253},"p2":{"x":397,"y":263},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp8994170676865566","type":"rectangle","data":{"p1":{"x":397,"y":253},"p2":{"x":407,"y":263},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp38981969516887605","type":"rectangle","data":{"p1":{"x":407,"y":253},"p2":{"x":417,"y":263},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp5668259350259238","type":"rectangle","data":{"p1":{"x":417,"y":253},"p2":{"x":427,"y":263},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp727218039283589","type":"rectangle","data":{"p1":{"x":427,"y":253},"p2":{"x":437,"y":263},"flipX":true},"style":{"fillColor":[184,233,134,1]}},{"id":"dp5855019033302965","type":"rectangle","data":{"p1":{"x":437,"y":253},"p2":{"x":447,"y":263},"flipX":true},"style":{"fillColor":[184,233,134,1]}}]},{"id":"dg9306880946329485","entities":[{"id":"dg9007691502540746","entities":[{"id":"dp8349499269832863","type":"rectangle","data":{"p1":{"x":417,"y":163},"p2":{"x":427,"y":173},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp30599322600932277","type":"rectangle","data":{"p1":{"x":427,"y":163},"p2":{"x":437,"y":173},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp804424676857019","type":"rectangle","data":{"p1":{"x":437,"y":163},"p2":{"x":447,"y":173},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp4088928021943734","type":"rectangle","data":{"p1":{"x":417,"y":173},"p2":{"x":427,"y":183},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp3991628996407597","type":"rectangle","data":{"p1":{"x":427,"y":173},"p2":{"x":437,"y":183},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp5528995521702358","type":"rectangle","data":{"p1":{"x":437,"y":173},"p2":{"x":447,"y":183},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp003022719959632769","type":"rectangle","data":{"p1":{"x":417,"y":183},"p2":{"x":427,"y":193},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp8459519253432544","type":"rectangle","data":{"p1":{"x":427,"y":183},"p2":{"x":437,"y":193},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp4243051581061511","type":"rectangle","data":{"p1":{"x":437,"y":183},"p2":{"x":447,"y":193},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp17296155933371693","type":"rectangle","data":{"p1":{"x":417,"y":193},"p2":{"x":427,"y":203},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp3826981261808039","type":"rectangle","data":{"p1":{"x":427,"y":193},"p2":{"x":437,"y":203},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp4983048931709224","type":"rectangle","data":{"p1":{"x":437,"y":193},"p2":{"x":447,"y":203},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp5546165868855052","type":"rectangle","data":{"p1":{"x":417,"y":203},"p2":{"x":427,"y":213},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp5159597222017771","type":"rectangle","data":{"p1":{"x":427,"y":203},"p2":{"x":437,"y":213},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp7318905437321647","type":"rectangle","data":{"p1":{"x":437,"y":203},"p2":{"x":447,"y":213},"flipX":true},"style":{"fillColor":[255,255,255,1]}}]},{"id":"dg4840414014672284","entities":[{"id":"dp32334995923258003","type":"rectangle","data":{"p1":{"x":417,"y":213},"p2":{"x":427,"y":223},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp7258754444437336","type":"rectangle","data":{"p1":{"x":427,"y":213},"p2":{"x":437,"y":223},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp34316875215154796","type":"rectangle","data":{"p1":{"x":437,"y":213},"p2":{"x":447,"y":223},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp04850036441198469","type":"rectangle","data":{"p1":{"x":417,"y":223},"p2":{"x":427,"y":233},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp8486830032532154","type":"rectangle","data":{"p1":{"x":427,"y":223},"p2":{"x":437,"y":233},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp2599927998257521","type":"rectangle","data":{"p1":{"x":437,"y":223},"p2":{"x":447,"y":233},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp3846296734014705","type":"rectangle","data":{"p1":{"x":417,"y":233},"p2":{"x":427,"y":243},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp9450258700463645","type":"rectangle","data":{"p1":{"x":427,"y":233},"p2":{"x":437,"y":243},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp12118570116984939","type":"rectangle","data":{"p1":{"x":437,"y":233},"p2":{"x":447,"y":243},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp8592990539195652","type":"rectangle","data":{"p1":{"x":417,"y":243},"p2":{"x":427,"y":253},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp1510070017949563","type":"rectangle","data":{"p1":{"x":427,"y":243},"p2":{"x":437,"y":253},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp5838385298434238","type":"rectangle","data":{"p1":{"x":437,"y":243},"p2":{"x":447,"y":253},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp9901992582853275","type":"rectangle","data":{"p1":{"x":417,"y":253},"p2":{"x":427,"y":263},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp8473152286015622","type":"rectangle","data":{"p1":{"x":427,"y":253},"p2":{"x":437,"y":263},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp7513748456017768","type":"rectangle","data":{"p1":{"x":437,"y":253},"p2":{"x":447,"y":263},"flipX":true},"style":{"fillColor":[255,255,255,1]}}]}]}]},{"id":"dg9950109222002476","entities":[{"id":"dp06624822890816318","type":"rectangle","data":{"p1":{"x":347,"y":25},"p2":{"x":357,"y":35},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp8439876460341093","type":"rectangle","data":{"p1":{"x":357,"y":25},"p2":{"x":367,"y":35},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp16291551372555502","type":"rectangle","data":{"p1":{"x":367,"y":25},"p2":{"x":377,"y":35},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp7937010654321652","type":"rectangle","data":{"p1":{"x":377,"y":25},"p2":{"x":387,"y":35},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp7094009850023141","type":"rectangle","data":{"p1":{"x":387,"y":25},"p2":{"x":397,"y":35},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp7695402277415495","type":"rectangle","data":{"p1":{"x":397,"y":25},"p2":{"x":407,"y":35},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp3333741075681975","type":"rectangle","data":{"p1":{"x":407,"y":25},"p2":{"x":417,"y":35},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp26055514642248656","type":"rectangle","data":{"p1":{"x":417,"y":25},"p2":{"x":427,"y":35},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp19450984173600394","type":"rectangle","data":{"p1":{"x":427,"y":25},"p2":{"x":437,"y":35},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp9499110230595194","type":"rectangle","data":{"p1":{"x":437,"y":25},"p2":{"x":447,"y":35},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dg8196174882319724","entities":[{"id":"dp7330544083671104","type":"rectangle","data":{"p1":{"x":347,"y":35},"p2":{"x":357,"y":45},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp5658537908269474","type":"rectangle","data":{"p1":{"x":357,"y":35},"p2":{"x":367,"y":45},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp9157950209123953","type":"rectangle","data":{"p1":{"x":367,"y":35},"p2":{"x":377,"y":45},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp7321569526857945","type":"rectangle","data":{"p1":{"x":377,"y":35},"p2":{"x":387,"y":45},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp8790888634760667","type":"rectangle","data":{"p1":{"x":387,"y":35},"p2":{"x":397,"y":45},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp7455316013484878","type":"rectangle","data":{"p1":{"x":397,"y":35},"p2":{"x":407,"y":45},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp5447502090491925","type":"rectangle","data":{"p1":{"x":407,"y":35},"p2":{"x":417,"y":45},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp4033534972479895","type":"rectangle","data":{"p1":{"x":417,"y":35},"p2":{"x":427,"y":45},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp8828338180596298","type":"rectangle","data":{"p1":{"x":427,"y":35},"p2":{"x":437,"y":45},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp8622280127833659","type":"rectangle","data":{"p1":{"x":437,"y":35},"p2":{"x":447,"y":45},"flipX":true},"style":{"fillColor":[120,164,216,1]}}]},{"id":"dg05109498740419527","entities":[{"id":"dp03747220562647913","type":"rectangle","data":{"p1":{"x":347,"y":45},"p2":{"x":357,"y":55},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp6967657293636924","type":"rectangle","data":{"p1":{"x":357,"y":45},"p2":{"x":367,"y":55},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp5595382047481579","type":"rectangle","data":{"p1":{"x":367,"y":45},"p2":{"x":377,"y":55},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp1763267147560562","type":"rectangle","data":{"p1":{"x":377,"y":45},"p2":{"x":387,"y":55},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp8933224284274208","type":"rectangle","data":{"p1":{"x":387,"y":45},"p2":{"x":397,"y":55},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp5380373364951707","type":"rectangle","data":{"p1":{"x":397,"y":45},"p2":{"x":407,"y":55},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp8456917022619855","type":"rectangle","data":{"p1":{"x":407,"y":45},"p2":{"x":417,"y":55},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp24113451225802773","type":"rectangle","data":{"p1":{"x":417,"y":45},"p2":{"x":427,"y":55},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp2257756668830896","type":"rectangle","data":{"p1":{"x":427,"y":45},"p2":{"x":437,"y":55},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp6257208282870468","type":"rectangle","data":{"p1":{"x":437,"y":45},"p2":{"x":447,"y":55},"flipX":true},"style":{"fillColor":[120,164,216,1]}}]},{"id":"dg5575306770120885","entities":[{"id":"dp6933950344547309","type":"rectangle","data":{"p1":{"x":347,"y":55},"p2":{"x":357,"y":65},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp6703453641912197","type":"rectangle","data":{"p1":{"x":357,"y":55},"p2":{"x":367,"y":65},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp09634876150931604","type":"rectangle","data":{"p1":{"x":367,"y":55},"p2":{"x":377,"y":65},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp9408648093639449","type":"rectangle","data":{"p1":{"x":377,"y":55},"p2":{"x":387,"y":65},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp8555456149043125","type":"rectangle","data":{"p1":{"x":387,"y":55},"p2":{"x":397,"y":65},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp8475827909655164","type":"rectangle","data":{"p1":{"x":397,"y":55},"p2":{"x":407,"y":65},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp16097523258160018","type":"rectangle","data":{"p1":{"x":407,"y":55},"p2":{"x":417,"y":65},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp1026001490375833","type":"rectangle","data":{"p1":{"x":417,"y":55},"p2":{"x":427,"y":65},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp5598558216462329","type":"rectangle","data":{"p1":{"x":427,"y":55},"p2":{"x":437,"y":65},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp8992023616064624","type":"rectangle","data":{"p1":{"x":437,"y":55},"p2":{"x":447,"y":65},"flipX":true},"style":{"fillColor":[120,164,216,1]}}]},{"id":"dg8229169949075518","entities":[{"id":"dp4621067178219712","type":"rectangle","data":{"p1":{"x":347,"y":65},"p2":{"x":357,"y":75},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp08980350590930819","type":"rectangle","data":{"p1":{"x":357,"y":65},"p2":{"x":367,"y":75},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp7009348423231776","type":"rectangle","data":{"p1":{"x":367,"y":65},"p2":{"x":377,"y":75},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp6451678751263022","type":"rectangle","data":{"p1":{"x":377,"y":65},"p2":{"x":387,"y":75},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp3169625612939635","type":"rectangle","data":{"p1":{"x":387,"y":65},"p2":{"x":397,"y":75},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp5114565790941878","type":"rectangle","data":{"p1":{"x":397,"y":65},"p2":{"x":407,"y":75},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp5099277177485139","type":"rectangle","data":{"p1":{"x":407,"y":65},"p2":{"x":417,"y":75},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp2553899389435048","type":"rectangle","data":{"p1":{"x":417,"y":65},"p2":{"x":427,"y":75},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp5451964561473787","type":"rectangle","data":{"p1":{"x":427,"y":65},"p2":{"x":437,"y":75},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp11642103585099728","type":"rectangle","data":{"p1":{"x":437,"y":65},"p2":{"x":447,"y":75},"flipX":true},"style":{"fillColor":[120,164,216,1]}}]},{"id":"dg5929396817345427","entities":[{"id":"dp4956972383907551","type":"rectangle","data":{"p1":{"x":347,"y":75},"p2":{"x":357,"y":85},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp505459494015787","type":"rectangle","data":{"p1":{"x":357,"y":75},"p2":{"x":367,"y":85},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp17511626677086045","type":"rectangle","data":{"p1":{"x":367,"y":75},"p2":{"x":377,"y":85},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp23569418498452432","type":"rectangle","data":{"p1":{"x":377,"y":75},"p2":{"x":387,"y":85},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp7835601005434033","type":"rectangle","data":{"p1":{"x":387,"y":75},"p2":{"x":397,"y":85},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp4269535403911102","type":"rectangle","data":{"p1":{"x":397,"y":75},"p2":{"x":407,"y":85},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp11874070227888878","type":"rectangle","data":{"p1":{"x":407,"y":75},"p2":{"x":417,"y":85},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp5245991958994425","type":"rectangle","data":{"p1":{"x":417,"y":75},"p2":{"x":427,"y":85},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp6184978348214899","type":"rectangle","data":{"p1":{"x":427,"y":75},"p2":{"x":437,"y":85},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp05596258961872691","type":"rectangle","data":{"p1":{"x":437,"y":75},"p2":{"x":447,"y":85},"flipX":true},"style":{"fillColor":[120,164,216,1]}}]},{"id":"dg8670774778758437","entities":[{"id":"dp4338391596158665","type":"rectangle","data":{"p1":{"x":347,"y":85},"p2":{"x":357,"y":95},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp9391621557788122","type":"rectangle","data":{"p1":{"x":357,"y":85},"p2":{"x":367,"y":95},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp6060012302312309","type":"rectangle","data":{"p1":{"x":367,"y":85},"p2":{"x":377,"y":95},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp026701766218797496","type":"rectangle","data":{"p1":{"x":377,"y":85},"p2":{"x":387,"y":95},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp6561021626332465","type":"rectangle","data":{"p1":{"x":387,"y":85},"p2":{"x":397,"y":95},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp7842704662517627","type":"rectangle","data":{"p1":{"x":397,"y":85},"p2":{"x":407,"y":95},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp26626332462575897","type":"rectangle","data":{"p1":{"x":407,"y":85},"p2":{"x":417,"y":95},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp9309370854086212","type":"rectangle","data":{"p1":{"x":417,"y":85},"p2":{"x":427,"y":95},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp135755847284332","type":"rectangle","data":{"p1":{"x":427,"y":85},"p2":{"x":437,"y":95},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp35077363666480565","type":"rectangle","data":{"p1":{"x":437,"y":85},"p2":{"x":447,"y":95},"flipX":true},"style":{"fillColor":[120,164,216,1]}}]},{"id":"dg710710919281675","entities":[{"id":"dp23238771852958273","type":"rectangle","data":{"p1":{"x":347,"y":95},"p2":{"x":357,"y":105},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp8623807242071061","type":"rectangle","data":{"p1":{"x":357,"y":95},"p2":{"x":367,"y":105},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp8465823096118698","type":"rectangle","data":{"p1":{"x":367,"y":95},"p2":{"x":377,"y":105},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp8340021929635831","type":"rectangle","data":{"p1":{"x":377,"y":95},"p2":{"x":387,"y":105},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp38326053658802595","type":"rectangle","data":{"p1":{"x":387,"y":95},"p2":{"x":397,"y":105},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp08417423234264276","type":"rectangle","data":{"p1":{"x":397,"y":95},"p2":{"x":407,"y":105},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp6809996847128087","type":"rectangle","data":{"p1":{"x":407,"y":95},"p2":{"x":417,"y":105},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp23725922039308733","type":"rectangle","data":{"p1":{"x":417,"y":95},"p2":{"x":427,"y":105},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp4699976873767562","type":"rectangle","data":{"p1":{"x":427,"y":95},"p2":{"x":437,"y":105},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp8299603387997121","type":"rectangle","data":{"p1":{"x":437,"y":95},"p2":{"x":447,"y":105},"flipX":true},"style":{"fillColor":[120,164,216,1]}}]},{"id":"dg7703643760375221","entities":[{"id":"dp8318207559704441","type":"rectangle","data":{"p1":{"x":347,"y":105},"p2":{"x":357,"y":115},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp5786623874536362","type":"rectangle","data":{"p1":{"x":357,"y":105},"p2":{"x":367,"y":115},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp550007453212728","type":"rectangle","data":{"p1":{"x":367,"y":105},"p2":{"x":377,"y":115},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp011116986580511856","type":"rectangle","data":{"p1":{"x":377,"y":105},"p2":{"x":387,"y":115},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp567823468622288","type":"rectangle","data":{"p1":{"x":387,"y":105},"p2":{"x":397,"y":115},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp41390456667606446","type":"rectangle","data":{"p1":{"x":397,"y":105},"p2":{"x":407,"y":115},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp34669291702079585","type":"rectangle","data":{"p1":{"x":407,"y":105},"p2":{"x":417,"y":115},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp12264920828070724","type":"rectangle","data":{"p1":{"x":417,"y":105},"p2":{"x":427,"y":115},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp7897636467767186","type":"rectangle","data":{"p1":{"x":427,"y":105},"p2":{"x":437,"y":115},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp047989083918181796","type":"rectangle","data":{"p1":{"x":437,"y":105},"p2":{"x":447,"y":115},"flipX":true},"style":{"fillColor":[120,164,216,1]}}]},{"id":"dg8780140626124295","entities":[{"id":"dp7678261344138662","type":"rectangle","data":{"p1":{"x":347,"y":115},"p2":{"x":357,"y":125},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp6493562511926297","type":"rectangle","data":{"p1":{"x":357,"y":115},"p2":{"x":367,"y":125},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp40583425975999143","type":"rectangle","data":{"p1":{"x":367,"y":115},"p2":{"x":377,"y":125},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp46225615359609507","type":"rectangle","data":{"p1":{"x":377,"y":115},"p2":{"x":387,"y":125},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp6120493456651793","type":"rectangle","data":{"p1":{"x":387,"y":115},"p2":{"x":397,"y":125},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp557297587636747","type":"rectangle","data":{"p1":{"x":397,"y":115},"p2":{"x":407,"y":125},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp02358886639571045","type":"rectangle","data":{"p1":{"x":407,"y":115},"p2":{"x":417,"y":125},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp5140334961888452","type":"rectangle","data":{"p1":{"x":417,"y":115},"p2":{"x":427,"y":125},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp686286416866523","type":"rectangle","data":{"p1":{"x":427,"y":115},"p2":{"x":437,"y":125},"flipX":true},"style":{"fillColor":[120,164,216,1]}},{"id":"dp6776847333342361","type":"rectangle","data":{"p1":{"x":437,"y":115},"p2":{"x":447,"y":125},"flipX":true},"style":{"fillColor":[120,164,216,1]}}]},{"id":"dg29847241967040605","entities":[{"id":"dp23059976766764667","type":"rectangle","data":{"p1":{"x":387,"y":25},"p2":{"x":397,"y":35},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp9475335957661445","type":"rectangle","data":{"p1":{"x":397,"y":25},"p2":{"x":407,"y":35},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp7737296628237831","type":"rectangle","data":{"p1":{"x":407,"y":25},"p2":{"x":417,"y":35},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp420552874032884","type":"rectangle","data":{"p1":{"x":417,"y":25},"p2":{"x":427,"y":35},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp0033472202146034302","type":"rectangle","data":{"p1":{"x":437,"y":25},"p2":{"x":447,"y":35},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp37598382409475595","type":"rectangle","data":{"p1":{"x":427,"y":25},"p2":{"x":437,"y":35},"flipX":true},"style":{"fillColor":[255,255,255,1]}}]},{"id":"dg12981550109624207","entities":[{"id":"dp2925621861374933","type":"rectangle","data":{"p1":{"x":387,"y":35},"p2":{"x":397,"y":45},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp4270624735565798","type":"rectangle","data":{"p1":{"x":397,"y":35},"p2":{"x":407,"y":45},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp6352215272969366","type":"rectangle","data":{"p1":{"x":407,"y":35},"p2":{"x":417,"y":45},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp5158856831055343","type":"rectangle","data":{"p1":{"x":417,"y":35},"p2":{"x":427,"y":45},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp5207213729430612","type":"rectangle","data":{"p1":{"x":437,"y":35},"p2":{"x":447,"y":45},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp2525406157953811","type":"rectangle","data":{"p1":{"x":427,"y":35},"p2":{"x":437,"y":45},"flipX":true},"style":{"fillColor":[255,255,255,1]}}]},{"id":"dg4516026449744355","entities":[{"id":"dp11715931756277098","type":"rectangle","data":{"p1":{"x":387,"y":45},"p2":{"x":397,"y":55},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp26713249938177996","type":"rectangle","data":{"p1":{"x":397,"y":45},"p2":{"x":407,"y":55},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp5530343515336709","type":"rectangle","data":{"p1":{"x":407,"y":45},"p2":{"x":417,"y":55},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp593474554265311","type":"rectangle","data":{"p1":{"x":417,"y":45},"p2":{"x":427,"y":55},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp9513255673947019","type":"rectangle","data":{"p1":{"x":437,"y":45},"p2":{"x":447,"y":55},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp6766373099320845","type":"rectangle","data":{"p1":{"x":427,"y":45},"p2":{"x":437,"y":55},"flipX":true},"style":{"fillColor":[255,255,255,1]}}]},{"id":"dg9233591108629413","entities":[{"id":"dp46821843584798395","type":"rectangle","data":{"p1":{"x":387,"y":55},"p2":{"x":397,"y":65},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp1346175523044011","type":"rectangle","data":{"p1":{"x":397,"y":55},"p2":{"x":407,"y":65},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp4701967337262757","type":"rectangle","data":{"p1":{"x":407,"y":55},"p2":{"x":417,"y":65},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp4572561926284904","type":"rectangle","data":{"p1":{"x":417,"y":55},"p2":{"x":427,"y":65},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp8145512947697867","type":"rectangle","data":{"p1":{"x":437,"y":55},"p2":{"x":447,"y":65},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp286924758607909","type":"rectangle","data":{"p1":{"x":427,"y":55},"p2":{"x":437,"y":65},"flipX":true},"style":{"fillColor":[255,255,255,1]}}]},{"id":"dg035143216759776386","entities":[{"id":"dp29769521308796054","type":"rectangle","data":{"p1":{"x":387,"y":65},"p2":{"x":397,"y":75},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp5087288450338762","type":"rectangle","data":{"p1":{"x":397,"y":65},"p2":{"x":407,"y":75},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp7755564676226789","type":"rectangle","data":{"p1":{"x":407,"y":65},"p2":{"x":417,"y":75},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp3791887210764203","type":"rectangle","data":{"p1":{"x":417,"y":65},"p2":{"x":427,"y":75},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp6664227131373087","type":"rectangle","data":{"p1":{"x":437,"y":65},"p2":{"x":447,"y":75},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp825461430674883","type":"rectangle","data":{"p1":{"x":427,"y":65},"p2":{"x":437,"y":75},"flipX":true},"style":{"fillColor":[255,255,255,1]}}]},{"id":"dg495148721185676","entities":[{"id":"dp3189302418494194","type":"rectangle","data":{"p1":{"x":387,"y":75},"p2":{"x":397,"y":85},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp4347183079002941","type":"rectangle","data":{"p1":{"x":397,"y":75},"p2":{"x":407,"y":85},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp3367011798678661","type":"rectangle","data":{"p1":{"x":407,"y":75},"p2":{"x":417,"y":85},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp42422666883584303","type":"rectangle","data":{"p1":{"x":417,"y":75},"p2":{"x":427,"y":85},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp8098217762194599","type":"rectangle","data":{"p1":{"x":437,"y":75},"p2":{"x":447,"y":85},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp6105630000221444","type":"rectangle","data":{"p1":{"x":427,"y":75},"p2":{"x":437,"y":85},"flipX":true},"style":{"fillColor":[255,255,255,1]}}]},{"id":"dg6372406400565114","entities":[{"id":"dp06389845772698688","type":"rectangle","data":{"p1":{"x":387,"y":75},"p2":{"x":397,"y":85},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp8062301441314433","type":"rectangle","data":{"p1":{"x":397,"y":75},"p2":{"x":407,"y":85},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp6284046106937419","type":"rectangle","data":{"p1":{"x":407,"y":75},"p2":{"x":417,"y":85},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp45510524155938104","type":"rectangle","data":{"p1":{"x":417,"y":75},"p2":{"x":427,"y":85},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp012255472140111023","type":"rectangle","data":{"p1":{"x":437,"y":75},"p2":{"x":447,"y":85},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp09042584577385027","type":"rectangle","data":{"p1":{"x":427,"y":75},"p2":{"x":437,"y":85},"flipX":true},"style":{"fillColor":[255,255,255,1]}}]},{"id":"dg8803598491287109","entities":[{"id":"dp13240228848927982","type":"rectangle","data":{"p1":{"x":387,"y":85},"p2":{"x":397,"y":95},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp8960800209414402","type":"rectangle","data":{"p1":{"x":397,"y":85},"p2":{"x":407,"y":95},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp6177681129352853","type":"rectangle","data":{"p1":{"x":407,"y":85},"p2":{"x":417,"y":95},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp7506683112489143","type":"rectangle","data":{"p1":{"x":417,"y":85},"p2":{"x":427,"y":95},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp6010413570661636","type":"rectangle","data":{"p1":{"x":437,"y":85},"p2":{"x":447,"y":95},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp42871109347338654","type":"rectangle","data":{"p1":{"x":427,"y":85},"p2":{"x":437,"y":95},"flipX":true},"style":{"fillColor":[255,255,255,1]}}]},{"id":"dg32163986735198646","entities":[{"id":"dp35187037539759025","type":"rectangle","data":{"p1":{"x":387,"y":95},"p2":{"x":397,"y":105},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp1133224252997228","type":"rectangle","data":{"p1":{"x":397,"y":95},"p2":{"x":407,"y":105},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp3657665386071337","type":"rectangle","data":{"p1":{"x":407,"y":95},"p2":{"x":417,"y":105},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp5916406249813053","type":"rectangle","data":{"p1":{"x":417,"y":95},"p2":{"x":427,"y":105},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp4273323755978444","type":"rectangle","data":{"p1":{"x":437,"y":95},"p2":{"x":447,"y":105},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp5488022918302613","type":"rectangle","data":{"p1":{"x":427,"y":95},"p2":{"x":437,"y":105},"flipX":true},"style":{"fillColor":[255,255,255,1]}}]},{"id":"dg1174963814637533","entities":[{"id":"dp17336212209270008","type":"rectangle","data":{"p1":{"x":387,"y":105},"p2":{"x":397,"y":115},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp6860442134568006","type":"rectangle","data":{"p1":{"x":397,"y":105},"p2":{"x":407,"y":115},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp8866237458865065","type":"rectangle","data":{"p1":{"x":407,"y":105},"p2":{"x":417,"y":115},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp23902594322019388","type":"rectangle","data":{"p1":{"x":417,"y":105},"p2":{"x":427,"y":115},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp7746745317772952","type":"rectangle","data":{"p1":{"x":437,"y":105},"p2":{"x":447,"y":115},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp5238808557025592","type":"rectangle","data":{"p1":{"x":427,"y":105},"p2":{"x":437,"y":115},"flipX":true},"style":{"fillColor":[255,255,255,1]}}]},{"id":"dg7725243254195246","entities":[{"id":"dp12541939884696296","type":"rectangle","data":{"p1":{"x":387,"y":115},"p2":{"x":397,"y":125},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp02447345660396172","type":"rectangle","data":{"p1":{"x":397,"y":115},"p2":{"x":407,"y":125},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp6962212968883169","type":"rectangle","data":{"p1":{"x":407,"y":115},"p2":{"x":417,"y":125},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp43760366031172804","type":"rectangle","data":{"p1":{"x":417,"y":115},"p2":{"x":427,"y":125},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp31559188406382777","type":"rectangle","data":{"p1":{"x":437,"y":115},"p2":{"x":447,"y":125},"flipX":true},"style":{"fillColor":[255,255,255,1]}},{"id":"dp44004628463788964","type":"rectangle","data":{"p1":{"x":427,"y":115},"p2":{"x":437,"y":125},"flipX":true},"style":{"fillColor":[255,255,255,1]}}]}]}],"settings":{"grid":true,"diagramHeight":356}}]}],"pageSettings":{"pageSize":{"width":1233,"sizeUnit":"px"}},"delayRenderCache":{"av":160,"map":{}},"___version":2,"version":2,"av":160}

==> figures/docs/9ddfd5e5-3692-49a4-a594-0dd353780949 <==
{"id":"321241621323","lines":[{"id":"n0.3851416450923924","blocks":[],"style":{"align":"center"}},{"blocks":[],"style":{"align":"center"},"id":"n0.8322566856058309"},{"id":"n0.43673328111520215","blocks":[{"id":"n0.5215228110888748","text":"\\diagram","type":"composite","elements":{"de07941907435049711":{"id":"de07941907435049711","lines":[{"id":"n0.693170493660951","blocks":[{"id":"n0.709597043836177","text":"validation error"}]}],"shape":{"data":{"p":{"x":42.38515062556206,"y":203.08288812326265},"rotation":269.58},"anchor":"left-top"},"isTextMode":true},"de5165939235821523":{"id":"de5165939235821523","lines":[{"blocks":[{"id":"n0.8787084052856935","text":"number of parameters"}],"id":"n0.5679743907736358"}],"shape":{"data":{"p":{"x":271.8901101763461,"y":276.5136679122193},"rotation":359.44},"anchor":"left-top"},"isTextMode":true}},"connections":[],"intersections":{"id":"di4044878697568992","items":[],"style":{}},"shapes":[{"id":"dp2774389125615092","type":"plot","data":{"p1":{"x":21,"y":10},"p2":{"x":641,"y":280}},"functions":[{"model":{"id":"n0.308337224148039","lines":[{"id":"n0.24169305216106407","blocks":[{"id":"n0.8363770339175434","text":"4 - 1 * log"},{"id":"n0.6835141640835477","type":"single","text":"("},{"text":"x - 2) ","id":"n0.206556821347057"}]}]},"style":{"strokeColor":[74,144,226,0.8],"thickness":2}}],"axes":{"xAxis":{"settings":{"axisThickness":1,"majorTextColor":[50,50,50],"axisColor":[50,50,50],"majorSteps":"auto","scale":20.823486328125,"plotAxisNumering":false,"minorTickShow":false,"plotAxisShow":true,"minorGridShow":false,"plotGridShow":true}},"yAxis":{"settings":{"axisThickness":1,"majorTextColor":[50,50,50],"axisColor":[50,50,50],"majorSteps":"auto","scale":20.823486328125,"plotAxisNumering":false}}},"variables":[],"settings":{"centerXDelta":62.733154296875,"centerYDelta":-21.678955078125}},{"id":"dp6341833671338676","type":"circle","data":{"p1":{"x":124,"y":137},"p2":{"x":136,"y":149}},"style":{"strokeColor":[74,144,226,1],"fillColor":[74,144,226,1]}},{"id":"dp2921228194646539","type":"circle","data":{"p1":{"x":199,"y":197},"p2":{"x":211,"y":209}},"style":{"strokeColor":[74,144,226,1],"fillColor":[74,144,226,1]}},{"id":"dp8951937777250725","type":"circle","data":{"p1":{"x":630,"y":235},"p2":{"x":642,"y":247}},"style":{"strokeColor":[74,144,226,1],"fillColor":[74,144,226,1]}},{"id":"dp7214280436273873","type":"circle","data":{"p1":{"x":367,"y":220},"p2":{"x":379,"y":232}},"style":{"strokeColor":[74,144,226,1],"fillColor":[74,144,226,1]}},{"id":"dg27250937622956484","entities":[{"id":"dp8127804900667018","type":"rectangle","data":{"p1":{"x":405.3311258278146,"y":112.93780687397708},"p2":{"x":455,"y":119.74058919803599}},"style":{"fillColor":[184,233,134,1]}},{"id":"dp6902925268815181","type":"rectangle","data":{"p1":{"x":405,"y":102},"p2":{"x":454.6688741721854,"y":108.80278232405891}},"style":{"fillColor":[120,164,216,1]}},{"id":"dp8004742760980953","type":"rectangle","data":{"p1":{"x":405,"y":155.35515548281506},"p2":{"x":454.6688741721854,"y":162.15793780687397}},"style":{"fillColor":[184,233,134,1]}},{"id":"dp31496900520650395","type":"rectangle","data":{"p1":{"x":405,"y":166.02618657937808},"p2":{"x":454.6688741721854,"y":172.828968903437}},"style":{"fillColor":[120,164,216,1]}},{"id":"dp17839332205358172","type":"rectangle","data":{"p1":{"x":405,"y":176.6972176759411},"p2":{"x":454.6688741721854,"y":183.5}},"style":{"fillColor":[184,233,134,1]}},{"id":"dp34786900280384947","type":"rectangle","data":{"p1":{"x":441.42384105960264,"y":176.6972176759411},"p2":{"x":455,"y":183.5}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp3277279046505368","type":"rectangle","data":{"p1":{"x":405.3311258278146,"y":123.6088379705401},"p2":{"x":455,"y":130.411620294599}},"style":{"fillColor":[120,164,216,1]}},{"id":"dp12149964612901865","type":"rectangle","data":{"p1":{"x":405.3311258278146,"y":134.2798690671031},"p2":{"x":455,"y":141.08265139116202}},"style":{"fillColor":[184,233,134,1]}},{"id":"dp6312101634320747","type":"rectangle","data":{"p1":{"x":405.3311258278146,"y":144.95090016366612},"p2":{"x":455,"y":151.75368248772503}},"style":{"fillColor":[120,164,216,1]}},{"id":"dp3484761887206256","type":"rectangle","data":{"p1":{"x":425.8609271523179,"y":102},"p2":{"x":454.6688741721854,"y":108.80278232405891}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp8221205391105307","type":"rectangle","data":{"p1":{"x":426.1920529801324,"y":123.6088379705401},"p2":{"x":455,"y":130.411620294599}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp1261762400141293","type":"rectangle","data":{"p1":{"x":426.1920529801324,"y":144.95090016366612},"p2":{"x":455,"y":151.75368248772503}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp12573532041245195","type":"rectangle","data":{"p1":{"x":425.8609271523179,"y":166.02618657937808},"p2":{"x":454.6688741721854,"y":172.828968903437}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp9835157295220961","type":"rectangle","data":{"p1":{"x":441.42384105960264,"y":112.93780687397708},"p2":{"x":455,"y":119.74058919803599}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp5366571971284052","type":"rectangle","data":{"p1":{"x":441.42384105960264,"y":134.2798690671031},"p2":{"x":455,"y":141.08265139116202}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp5174795829207886","type":"rectangle","data":{"p1":{"x":441.09271523178813,"y":155.35515548281506},"p2":{"x":454.6688741721854,"y":162.15793780687397}},"style":{"fillColor":[255,255,255,1]}}],"data":{}},{"id":"dg3897079010725527","entities":[{"id":"dp7762607745726143","type":"rectangle","data":{"p1":{"x":560,"y":138.10556464811785},"p2":{"x":623,"y":144.86661211129294}},"style":{"fillColor":[184,233,134,1]}},{"id":"dp08493070025180438","type":"rectangle","data":{"p1":{"x":560,"y":127.5},"p2":{"x":623,"y":134.26104746317512}},"style":{"fillColor":[120,164,216,1]}},{"id":"dp7084401556724232","type":"rectangle","data":{"p1":{"x":560,"y":148.7111292962357},"p2":{"x":623,"y":155.4721767594108}},"style":{"fillColor":[120,164,216,1]}},{"id":"dp3001518937920109","type":"rectangle","data":{"p1":{"x":560,"y":159.31669394435352},"p2":{"x":623,"y":166.07774140752863}},"style":{"fillColor":[184,233,134,1]}},{"id":"dp3626540284970783","type":"rectangle","data":{"p1":{"x":560,"y":180.5278232405892},"p2":{"x":623,"y":187.2888707037643}},"style":{"fillColor":[184,233,134,1]}},{"id":"dp3937186879406913","type":"rectangle","data":{"p1":{"x":560,"y":169.92225859247137},"p2":{"x":623,"y":176.68330605564648}},"style":{"fillColor":[120,164,216,1]}},{"id":"dp5838058379007223","type":"rectangle","data":{"p1":{"x":560,"y":191.13338788870703},"p2":{"x":623,"y":197.89443535188215}},"style":{"fillColor":[120,164,216,1]}},{"id":"dp9795451920191779","type":"rectangle","data":{"p1":{"x":560,"y":201.73895253682485},"p2":{"x":623,"y":208.5}},"style":{"fillColor":[184,233,134,1]}}],"data":{}},{"id":"da758989420405923","data":[{"x":273,"y":153.5},{"x":212,"y":195}],"head":">","tail":"no","shaft":"-","mVer":1,"style":{"thickness":3}},{"id":"da029623408881354174","data":[{"x":401,"y":192.5},{"x":380,"y":219}],"head":">","tail":"no","shaft":"-","mVer":1,"style":{"thickness":3}},{"id":"da44154551298249767","data":[{"x":590,"y":212.5},{"x":622,"y":232.5}],"head":">","tail":"no","shaft":"-","mVer":1,"style":{"thickness":3}},{"id":"dg47941653929841965","entities":[{"id":"dp32013032102270234","type":"rectangle","data":{"p1":{"x":154.42384105960275,"y":24.47431726082104},"p2":{"x":218,"y":31.61078287425849}},"style":{"fillColor":[184,233,134,1]}},{"id":"dp3099376921477299","type":"rectangle","data":{"p1":{"x":154,"y":13},"p2":{"x":217.57615894039733,"y":20.13646561343745}},"style":{"fillColor":[120,164,216,1]}},{"id":"dp7243231923126666","type":"rectangle","data":{"p1":{"x":154,"y":68.9722793210783},"p2":{"x":217.57615894039733,"y":76.10874493451578}},"style":{"fillColor":[184,233,134,1]}},{"id":"dp14702314945409622","type":"rectangle","data":{"p1":{"x":154,"y":80.16673518529399},"p2":{"x":217.57615894039733,"y":87.30320079873144}},"style":{"fillColor":[120,164,216,1]}},{"id":"dp7129887948383195","type":"rectangle","data":{"p1":{"x":154,"y":91.36119104950959},"p2":{"x":217.57615894039733,"y":98.49765666294707}},"style":{"fillColor":[184,233,134,1]}},{"id":"dp9876447478207596","type":"rectangle","data":{"p1":{"x":154.42384105960275,"y":35.668773125036694},"p2":{"x":218,"y":42.8052387384742}},"style":{"fillColor":[120,164,216,1]}},{"id":"dp7803269083433821","type":"rectangle","data":{"p1":{"x":154.42384105960275,"y":46.86322898925232},"p2":{"x":218,"y":53.99969460268983}},"style":{"fillColor":[184,233,134,1]}},{"id":"dp6560815141733731","type":"rectangle","data":{"p1":{"x":154.42384105960275,"y":58.057684853468004},"p2":{"x":218,"y":65.19415046690548}},"style":{"fillColor":[120,164,216,1]}},{"id":"dp3967073789371778","type":"rectangle","data":{"p1":{"x":154,"y":13},"p2":{"x":217.57615894039733,"y":20.13646561343745}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp37676160380689916","type":"rectangle","data":{"p1":{"x":154.42384105960275,"y":24.47431726082104},"p2":{"x":218,"y":31.61078287425849}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp7877614171103046","type":"rectangle","data":{"p1":{"x":154.42384105960275,"y":35.64634404181592},"p2":{"x":218,"y":42.8052387384742}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp067109369740049","type":"rectangle","data":{"p1":{"x":154.42384105960275,"y":58.057684853468004},"p2":{"x":218,"y":65.19415046690548}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp6841111816305538","type":"rectangle","data":{"p1":{"x":170.5,"y":80.16673518529399},"p2":{"x":217.57615894039733,"y":87.27513966480447}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp3122108892358796","type":"rectangle","data":{"p1":{"x":154.42384105960275,"y":46.86088565219944},"p2":{"x":218,"y":53.99969460268983}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp21430246282294796","type":"rectangle","data":{"p1":{"x":154,"y":68.9722793210783},"p2":{"x":217.57615894039733,"y":76.10874493451578}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp6397097019134936","type":"rectangle","data":{"p1":{"x":190,"y":91.36119104950959},"p2":{"x":217.57615894039733,"y":98.5}},"style":{"fillColor":[255,255,255,1]}}],"data":{}},{"id":"dg05906033507137842","entities":[{"id":"dp5200527352860257","type":"rectangle","data":{"p1":{"x":284.3973509933776,"y":67.66910201444765},"p2":{"x":344,"y":74.30476302343334}},"style":{"fillColor":[184,233,134,1]}},{"id":"dp47054130966068086","type":"rectangle","data":{"p1":{"x":284,"y":57},"p2":{"x":343.6026490066225,"y":63.63566100898572}},"style":{"fillColor":[120,164,216,1]}},{"id":"dp3496940883429178","type":"rectangle","data":{"p1":{"x":284,"y":109.04440007047631},"p2":{"x":343.6026490066225,"y":115.68006107946204}},"style":{"fillColor":[184,233,134,1]}},{"id":"dp4712611144012525","type":"rectangle","data":{"p1":{"x":284,"y":119.45328008457159},"p2":{"x":343.6026490066225,"y":126.08894109355731}},"style":{"fillColor":[120,164,216,1]}},{"id":"dp5001311223317141","type":"rectangle","data":{"p1":{"x":284,"y":129.8621600986668},"p2":{"x":343.6026490066225,"y":136.49782110765253}},"style":{"fillColor":[184,233,134,1]}},{"id":"dp2772055405419842","type":"rectangle","data":{"p1":{"x":284.3973509933776,"y":78.07798202854289},"p2":{"x":344,"y":84.71364303752864}},"style":{"fillColor":[120,164,216,1]}},{"id":"dp8399293897661312","type":"rectangle","data":{"p1":{"x":284.3973509933776,"y":88.48686204263814},"p2":{"x":344,"y":95.12252305162389}},"style":{"fillColor":[184,233,134,1]}},{"id":"dp9318779552959283","type":"rectangle","data":{"p1":{"x":284.3973509933776,"y":98.89574205673338},"p2":{"x":344,"y":105.53140306571913}},"style":{"fillColor":[120,164,216,1]}},{"id":"dp05476543414662527","type":"rectangle","data":{"p1":{"x":284,"y":57},"p2":{"x":343.60264900662247,"y":63.63566100898572}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp24836332584275733","type":"rectangle","data":{"p1":{"x":284.3973509933776,"y":67.66910201444765},"p2":{"x":344,"y":74.30476302343334}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp9295540699070384","type":"rectangle","data":{"p1":{"x":284.3973509933776,"y":78.05712691607445},"p2":{"x":344,"y":84.71364303752864}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp267155862331352","type":"rectangle","data":{"p1":{"x":304.39735099337753,"y":98.89574205673338},"p2":{"x":344,"y":105.55225817818757}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp6285699726425817","type":"rectangle","data":{"p1":{"x":304,"y":119.45328008457159},"p2":{"x":343.6026490066225,"y":126.10979620602572}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp0567185015772268","type":"rectangle","data":{"p1":{"x":284.3973509933776,"y":88.48468315029072},"p2":{"x":344,"y":95.12252305162389}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp5968968613081211","type":"rectangle","data":{"p1":{"x":311.48997295028437,"y":109.04440007047631},"p2":{"x":343.6026490066225,"y":115.68223997180948}},"style":{"fillColor":[255,255,255,1]}},{"id":"dp831586408854438","type":"rectangle","data":{"p1":{"x":311.48997295028437,"y":129.8621600986668},"p2":{"x":343.6026490066225,"y":136.5}},"style":{"fillColor":[255,255,255,1]}}],"data":{}},{"id":"da8695386176166314","data":[{"x":164,"y":105},{"x":136,"y":143}],"head":">","tail":"no","shaft":"-","mVer":1,"style":{"thickness":3}}],"settings":{"grid":false,"diagramHeight":310}}]},{"blocks":[{"text":"\\diagram","type":"composite","elements":{},"connections":[],"intersections":{"id":"di4044878697568992","items":[],"style":{}},"shapes":[],"settings":{"grid":false,"diagramHeight":310},"id":"n0.5904521710511554"}],"id":"n0.13206222574995619"}],"pageSettings":{"pageSize":{"width":700},"printedPageSize":{"presetSize":"letter","width":8.27,"height":11.69,"sizeUnit":"inch","orientation":"portrait","margin":{"left":1,"top":1,"right":1,"bottom":1,"unit":"inch"},"headerFooterModel":{"header":[{"id":"n0.8765652569343332","blocks":[]}],"footer":[{"id":"n0.3321572066226297","blocks":[]}]}}},"delayRenderCache":{"av":378,"map":{}},"___version":2,"version":2,"av":378}
